Leveraging Angle of Arrival Estimation against Impersonation Attacks in Physical Layer Authentication

In this paper, we investigate the utilization of the angle of arrival (AoA) as a feature for robust physical layer authentication (PLA). While most of the existing approaches to PLA focus on common features of the physical layer of communication channels, such as channel frequency response, channel impulse response or received signal strength, the use of AoA in this domain has not yet been studied in depth, particularly regarding the ability to thwart impersonation attacks. In this work, we demonstrate that an impersonation attack targeting AoA based PLA is only feasible under strict conditions on the attacker's location and hardware capabilities, which highlights the AoA's potential as a strong feature for PLA. We extend previous works considering a single-antenna attacker to the case of a multiple-antenna attacker, and we develop a theoretical characterization of the conditions in which a successful impersonation attack can be mounted. Furthermore, we leverage extensive simulations in support of theoretical analyses, to validate the robustness of AoA-based PLA.

==> Figures/MSE_vs_L_prova.tex <==


% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.00000,0.44706,0.74118}%
\definecolor{mycolor6}{rgb}{0.85098,0.32549,0.09804}%
\definecolor{mycolor7}{rgb}{0.92941,0.69412,0.12549}%
\definecolor{mycolor8}{rgb}{0.49412,0.18431,0.55686}%
%
\begin{tikzpicture}[scale=0.7\columnwidth/10cm,font=\footnotesize]

\begin{axis}[%
width=4.514in,
height=3.566in,
at={(0.757in,0.481in)},
scale only axis,
xmin=1,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={L},
ymin=0,
ymax=4,
ylabel style={font=\color{white!15!black}},
ylabel={MSE},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black, fill opacity=0.8}
]
\addplot [color=mycolor1, line width=1.5pt]
  table[row sep=crcr]{%
1	1.98368254701479\\
2	1.9982174744615\\
3	1.98892707107522\\
4	2.00358919162647\\
5	2.00647783228177\\
6	2.0044268186195\\
7	2.00325501813398\\
8	1.99378253790233\\
9	1.96145494867092\\
10	1.99488214801423\\
11	2.00447612625464\\
12	2.01978888103866\\
13	2.02579518340653\\
14	2.02427904876463\\
15	1.99190185459215\\
16	1.99423920881331\\
17	1.99677323789756\\
18	2.01092549620386\\
19	2.0084281148137\\
20	1.99400083534083\\
};
\addlegendentry{SNR = 0 dB, $\hat{\theta_0} = 0.4$}

\addplot [color=mycolor2, line width=1.5pt]
  table[row sep=crcr]{%
1	0.640120830556421\\
2	0.636071187192649\\
3	0.627322629491098\\
4	0.627668601188635\\
5	0.626136404573387\\
6	0.623385643448471\\
7	0.6327996619683\\
8	0.631623361910528\\
9	0.638917379183566\\
10	0.639197471967084\\
11	0.627261796652028\\
12	0.630591156273247\\
13	0.622405407314562\\
14	0.639708256061868\\
15	0.638823519325414\\
16	0.629603825171973\\
17	0.623966199195377\\
18	0.62949054711245\\
19	0.632285280072989\\
20	0.62757903549033\\
};
\addlegendentry{SNR = 5 dB, $\hat{\theta_0} = 0.4$}

\addplot [color=mycolor3, line width=1.5pt]
  table[row sep=crcr]{%
1	0.199456770459934\\
2	0.201985062539138\\
3	0.200712463796152\\
4	0.202872655769708\\
5	0.200083908858062\\
6	0.19669597922522\\
7	0.198232857532692\\
8	0.19989531355567\\
9	0.199080210196368\\
10	0.201357658156838\\
11	0.198791118678885\\
12	0.199453450408733\\
13	0.200063468522637\\
14	0.202785864516839\\
15	0.202502882531945\\
16	0.200103864417382\\
17	0.195774164054451\\
18	0.200427775022384\\
19	0.201457118219867\\
20	0.198275304868367\\
};
\addlegendentry{SNR = 10 dB, $\hat{\theta_0} = 0.4$}

\addplot [color=mycolor4, line width=1.5pt]
  table[row sep=crcr]{%
1	0.0196199070350918\\
2	0.0198936694516894\\
3	0.0201797561987533\\
4	0.0202966241091176\\
5	0.0200302832259876\\
6	0.019815570547172\\
7	0.0201695531559291\\
8	0.0200963492831578\\
9	0.0198395943494748\\
10	0.0204285071951545\\
11	0.0199759437053935\\
12	0.0199235959938779\\
13	0.0202460603542615\\
14	0.0198899035913029\\
15	0.0195704097011771\\
16	0.0197960385936435\\
17	0.0202736840728829\\
18	0.0198501317189031\\
19	0.0198263162625973\\
20	0.0195649769162978\\
};
\addlegendentry{SNR = 20 dB, $\hat{\theta_0} = 0.4$}

\addplot [color=mycolor5, dashed, line width=1.5pt]
  table[row sep=crcr]{%
1	3.61059840742267\\
2	3.60902480688066\\
3	3.58615769488291\\
4	3.5856643291724\\
5	3.58690698113791\\
6	3.60051487408405\\
7	3.56508230540421\\
8	3.61606926555262\\
9	3.57398917636993\\
10	3.57998646727195\\
11	3.5626823357361\\
12	3.63612590270696\\
13	3.55164465564401\\
14	3.57074553371176\\
15	3.60611396639057\\
16	3.59988573049076\\
17	3.60280549748487\\
18	3.56996092718418\\
19	3.57253485236285\\
20	3.57767578723059\\
};
\addlegendentry{SNR = 0 dB, $\hat{\theta_0} = 0.5$}

\addplot [color=mycolor6, dashed, line width=1.5pt]
  table[row sep=crcr]{%
1	2.20063517552245\\
2	2.21719845482047\\
3	2.21778398925229\\
4	2.23843415532533\\
5	2.19454374977817\\
6	2.20834534375453\\
7	2.2539926137688\\
8	2.23044697337398\\
9	2.24110666353082\\
10	2.22803148592723\\
11	2.19971162791572\\
12	2.23284303548779\\
13	2.23707392932477\\
14	2.21752064328168\\
15	2.23265473221548\\
16	2.2192595337364\\
17	2.19324449523158\\
18	2.24516894934969\\
19	2.18459181997175\\
20	2.23275328760417\\
};
\addlegendentry{SNR = 5 dB, $\hat{\theta_0} = 0.5$}

\addplot [color=mycolor7, dashed, line width=1.5pt]
  table[row sep=crcr]{%
1	1.79127410799278\\
2	1.76980533440799\\
3	1.77804307118089\\
4	1.80843142666052\\
5	1.79562334721487\\
6	1.78505020218421\\
7	1.7928510516949\\
8	1.76234801791401\\
9	1.76898782460153\\
10	1.79730409149694\\
11	1.76698087345109\\
12	1.80073446283685\\
13	1.77594240709047\\
14	1.78985259534076\\
15	1.81296624772744\\
16	1.79254747529643\\
17	1.77662687989803\\
18	1.76429488752201\\
19	1.81155337596069\\
20	1.80202754133554\\
};
\addlegendentry{SNR = 10 dB, $\hat{\theta_0} = 0.5$}

\addplot [color=mycolor8, dashed, line width=1.5pt]
  table[row sep=crcr]{%
1	1.60356628361152\\
2	1.62700913027985\\
3	1.61040280565583\\
4	1.59844750177787\\
5	1.61342443838458\\
6	1.6205703889859\\
7	1.60221367054932\\
8	1.60524035900592\\
9	1.61070424372591\\
10	1.60428329887548\\
11	1.5979765012818\\
12	1.56736620282708\\
13	1.61257661540975\\
14	1.59758734527721\\
15	1.62166704594379\\
16	1.58022448095488\\
17	1.5834039925307\\
18	1.62569640047602\\
19	1.60286371285363\\
20	1.59897853954444\\
};
\addlegendentry{SNR = 20 dB, $\hat{\theta_0} = 0.5$}

\end{axis}

\begin{axis}[%
width=5.825in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%


